From Generation to Judgment: Opportunities and Challenges of LLM-as-a-judge

Assessment and evaluation have long been critical challenges in artificial intelligence (AI) and natural language processing (NLP). Traditional methods, usually matching-based or small model-based, often fall short in open-ended and dynamic scenarios. Recent advancements in Large Language Models (LLMs) inspire the "LLM-as-a-judge" paradigm, where LLMs are leveraged to perform scoring, ranking, or selection for various machine learning evaluation scenarios. This paper presents a comprehensive survey of LLM-based judgment and assessment, offering an in-depth overview to review this evolving field. We first provide the definition from both input and output perspectives. Then we introduce a systematic taxonomy to explore LLM-as-a-judge along three dimensions: what to judge, how to judge, and how to benchmark. Finally, we also highlight key challenges and promising future directions for this emerging area. More resources on LLM-as-a-judge are on the website: https://llm-as-a-judge.github.io and https://github.com/llm-as-a-judge/Awesome-LLM-as-a-judge.

==> tree1.tex <==
\tikzstyle{my-box}= [
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=pink!60, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep
=4pt,
]
\begin{figure*}[h!]

    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=4.5em,font=\scriptsize,}{},
            where level=2{text width=5.7em,font=\scriptsize,}{},
            where level=3{text width=6.4em,font=\scriptsize,}{},
            where level=4{text width=6.4em,font=\scriptsize,}{},
            [
        LLM-as-a-judge, ver
        [
    Attribute (\S \ref{Attributes})
    [
        Helpfulness (\S \ref{Helpfulness})
        [
            E.g.: Constitutional AI~\cite{bai2022constitutional}{, }RLAIF~\cite{lee2023rlaif}{, }MT-Bench~\cite{zheng2023judging}{, }Just-Eval~\cite{lin2023unlocking}{, }Starling~\cite{zhu2024starling}, leaf, text width=41em
        ]
    ]
    [
        Harmlessness (\S \ref{Harmlessness})
        [
            E.g.: LLaMA Guard~\cite{inan2023llama}{, }TRUSTGPT~\cite{huang2023trustgpt}{, }Moral Choice~\cite{scherrer2024evaluating}{, }
            SORRY-Bench~\cite{xie2024sorry}, leaf, text width=41em
        ]
    ]
    [
        Reliability (\S \ref{Reliability})
        [
            E.g.: FactScore~\cite{min2023factscore}{, }HALU-J~\cite{wang2024halu}{, }HalluJudge~\cite{luo2024halludial}{, }HalluQA~\cite{cheng2023evaluating}{, }
            SaySelf~\cite{xu2024sayself}, leaf, text width=41em
        ]
    ]
    [
        Relevance (\S \ref{Relevance})
        [
            E.g.: LLM-Eval~\cite{lin2023llm}{, }MoT~\cite{li-qiu-2023-mot}{, }~\cite{abbasiantaeb2024can}{, }
            DALK~\cite{li2024dalk}{, }MJ-Bench~\cite{chen2024mj}, leaf, text width=41em
        ]
    ]
    [
        Feasibility (\S \ref{Feasibility})
        [
            E.g.: RAP~\cite{hao2023reasoning}{, }ToT~\cite{yao2023tree}{, }Auto-GPT~\cite{yang2023auto}{, }GoT~\cite{besta2024graph}{, }Diffagent~\cite{zhao2024diffagent}, leaf, text width=41em
        ]
    ]
    [
        Overall Quality (\S \ref{Overall Quality})
        [
           E.g.: \cite{gao2023human}{, }Just-Eval~\cite{lin2023unlocking}{, }ICE~\cite{Jain2023MultiDimensionalEO}{, }LLM-Eval~\cite{Lin2023LLMEvalUM}{, }GEMBA~\cite{Kocmi2023LargeLM}{, }, leaf, text width=41em
        ]
    ]
]
        [
    Methodology (\S \ref{Methodology})
    [
        Tuning (\S \ref{Tuning})
        [
            Data Source\\ (\S \ref{Data Source})
            [
                Manually-labeled
                [
                    E.g.: AttrScore~\cite{yue2023automatic}{, }
                    PandaLM~\cite{wang2024pandalm}{, }
                    X-Eval~\cite{liu2024x}{, }, leaf, text width=25em
                ]
            ]
            [
                Synthetic Feedback
                [
                    E.g.: JudgeLM~\cite{zhu2023judgelm}{, }
                    AUTO-J~\cite{li2024generative}{, }
                    HALU-J ~\cite{wang2024halu}, leaf, text width=25em
                ]
            ]
        ]
        [
            Tuning Techniques\\ (\S \ref{Tuning Techniques})
            [
                Supervised Fine-Tuning
                [
                    E.g.: PerSE~\cite{wang2023learning}{, }
                    JudgeLM~\cite{zhu2023judgelm}{, }
                    X-Eval~\cite{liu2024x}, leaf, text width=25em
                ]
            ]
            [
                Preference Learning
                [
                    E.g.: HALU-J~\cite{wang2024halu}{, }
                    PORTIA\cite{li2024split}{, }
                    Themis~\cite{hu2024themis}
                    , leaf, text width=25em
                ]
            ]
        ]
    ]
    [
        Prompting (\S \ref{Prompting})
        [
            Swapping Operation\\ (\S \ref{swapping})
            [
                E.g.: MT-Bench~\cite{zheng2023judging}{, }
                RLAIF~\cite{lee2023rlaif}{, }
                SALMON~\cite{sun2024salmon}{, }Self-Judge~\cite{lee2024aligning}{, }\\Starling~\cite{zhu2024starling}, leaf, text width=33em
            ]
        ]
        [
            Rule Augmentation\\ (\S \ref{rule})
            [
                 E.g.: Constitutional AI~\cite{bai2022constitutional}{, }
                 MoT~\cite{li-qiu-2023-mot}{, }
               \cite{lahoti2023improving}{, }
                RLAIF~\cite{lee2023rlaif}{, }\\
                LRQ-Fact\cite{beigi2024lrq}{, }
                AUTO-J~\cite{li2024generative}{, }
               \cite{bai2024benchmarking}{, }       
                \cite{gao2023human}{, }
                Prometheus~\cite{kim2023prometheus}, leaf, text width=33em
            ]
        ]
        [
            Multi-Agent \\Collaboration (\S \ref{multi})
            [
                E.g.: PRD~\cite{li2023prd}{, }
               \cite{zhang2023wider}{, }
               \cite{wu2023large}{, }
                MPA~\cite{zhu2024dynamic}{, }
                JudgeLM~\cite{zhu2023judgelm}{, }\\
                ChatEval\cite{chanchateval}{, } 
                CoEvol~\cite{li2024coevol}
                LRQ-Fact~\cite{beigi2024lrq}{, }
                Cascaded Selection~\cite{jung2024trust}, leaf, text width=33em
            ]
        ]
        [
            Demonstration (\S \ref{demon})
            [
                E.g.: ICE~\cite{jain2023multi}{, }
                Little Giants~\cite{kotonya2023little}{, }
                ALLURE~\cite{hasanbeig2023allure}, leaf, text width=33em
            ]
        ]
        [
            Multi-Turn Interaction \\ (\S \ref{multiturn})
            [
                E.g.: LLM-as-an-examine~\cite{bai2023benchmarking}{, }
                KIEVAL~\cite{yu2024kieval}{, }
                Auto-Arena~\cite{zhao2024auto}{, }\\
               \cite{moniri2024evaluating}, leaf, text width=33em
            ]
        ]
        [
            Comparison\\ Acceleration (\S \ref{compare})
            [
                E.g.: \cite{liu2023statistical}{, }
                OSP~\cite{zhai2024online}{, }
                Starling~\cite{zhu2024starling}{, }
                Self-Judge~\cite{lee2024aligning}, leaf, text width=33em
            ]
        ]
    ]
]
        [
    Application (\S \ref{Application})
    [
        Evaluation (\S \ref{Evaluation})
        [
           E.g.: \cite{bi2023oceangpt}{, }\cite{fei2023lawbench}{, }\cite{zhou2023sotopia}{, }\cite{wang2023can}{, }\cite{nan2023evaluating}{, }\cite{zheng2023judging}{, }\cite{gao2023human}, leaf, text width=41em
        ]
    ]
    [
        Alignment (\S \ref{Alignment})
        [
           E.g.: \cite{bai2022constitutional}{, }\cite{lee2023rlaif}{, }\cite{sun2024salmon}{, }\cite{guo2024direct}{, }\cite{arif2024fellowship}{, }\cite{li2024coevol}{, }\cite{yuan2024self}{, }, leaf, text width=41em
        ]
    ]
    [
        Retrieval (\S \ref{Retrieval})
        [
           E.g.: \cite{sun2023chatgpt}{, }\cite{thomas2023large}{, }\cite{ma2023zero}{, }\cite{tang2024found}{, }\cite{qin2024large}{, }\cite{ma2024leveraging}{, }\cite{hou2024large}, leaf, text width=41em
        ]
    ]
    [
        Reasoning (\S \ref{reasoning})
        [
            E.g.: \cite{yao2022react}{, }\cite{creswell2022selection}{, }\cite{wei2022chain}{, }\cite{yao2023tree}{, }\cite{yang2023auto}{, }\cite{sha2023languagempc}{, }\cite{hao2023reasoning}{, }, leaf, text width=41em
        ]
    ]
]
    ]
        \end{forest}
    }
    \caption{Taxonomy of research in LLM-as-a-judge that consists of judging attribute, methodology, and application.}
    \label{categorization_of_reasoning}
    \vspace{-1mm}
\end{figure*}
